Towards Relation Extraction From Speech

Relation extraction typically aims to extract semantic relationships between entities from the unstructured text. One of the most essential data sources for relation extraction is the spoken language, such as interviews and dialogues. However, the error propagation introduced in automatic speech recognition (ASR) has been ignored in relation extraction, and the end-to-end speech-based relation extraction method has been rarely explored. In this paper, we propose a new listening information extraction task, i.e., speech relation extraction. We construct the training dataset for speech relation extraction via text-to-speech systems, and we construct the testing dataset via crowd-sourcing with native English speakers. We explore speech relation extraction via two approaches: the pipeline approach conducting text-based extraction with a pretrained ASR module, and the end2end approach via a new proposed encoder-decoder model, or what we called SpeechRE. We conduct comprehensive experiments to distinguish the challenges in speech relation extraction, which may shed light on future explorations. We share the code and data on https://github.com/wutong8023/SpeechRE.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/table/ERT.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\multirow{2}{*}{Decoding}      & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Entity} & \multicolumn{3}{c}{Relation} & \multicolumn{3}{c}{Triplet} \\ \cmidrule(l){3-11} 
                               &                         & Precision & Recall & F1    & Precision  & Recall  & F1    & Precision  & Recall & F1    \\ \midrule
\multirow{3}{*}{Unconstrained} & REBEL (Text)            & 99.99     & 99.99  & 99.99 & 99.99      & 99.99   & 99.99 & 99.99      & 99.99  & 99.99 \\
                               & REBEL (Transcript)      & 99.99     & 99.99  & 99.99 & 99.99      & 99.99   & 99.99 & 99.99      & 99.99  & 99.99 \\
                               & SpeechRE                & 99.99     & 99.99  & 99.99 & 99.99      & 99.99   & 99.99 & 99.99      & 99.99  & 99.99 \\ \midrule
\multirow{3}{*}{Entity-forced} & REBEL (Text)            & \_        & \_     & \_    & 99.99      & 99.99   & 99.99 & \_         & \_     & \_    \\
                               & REBEL (Transcript)      & \_        & \_     & \_    & 99.99      & 99.99   & 99.99 & \_         & \_     & \_    \\
                               & SpeechRE                & \_        & \_     & \_    & 99.99      & 99.99   & 99.99 & \_         & \_     & \_    \\ \bottomrule
\end{tabular}}
\caption{The evaluation of triplet extraction on entity recognition and relation classification.}
\label{tab:ert}
\end{table*}

==> section/table/entity_accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{@{}|c|c|cccccc|cccccc|@{}}
\toprule
                                             &                         & \multicolumn{6}{c|}{Multi   Speaker}                                                                                                                                                                                                                                                                   & \multicolumn{6}{c|}{Pseudo   Labeling}                                                                                                                                                                                                                                                                 \\ \cmidrule(l){3-14} 
\multirow{-2}{*}{Entity}                     & \multirow{-2}{*}{Total} & \multicolumn{1}{c|}{100\%}                         & \multicolumn{1}{c|}{100\% + 50\%}                  & \multicolumn{1}{c|}{100\% + 100\%}                 & \multicolumn{1}{c|}{100\% + 150\%}                 & \multicolumn{1}{c|}{100\% + 200\%}                 & 100\% + 250\%                 & \multicolumn{1}{c|}{100\%}                         & \multicolumn{1}{c|}{100\% + 50\%}                  & \multicolumn{1}{c|}{100\% + 100\%}                 & \multicolumn{1}{c|}{100\% + 150\%}                 & \multicolumn{1}{c|}{100\% + 200\%}                 & 100\% + 250\%                 \\ \midrule
Amanda Knox                                  & 4                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{D2EBDB}25}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{A8DAB7}50    \\ \midrule
Ahmed Rashid                                 & 6                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{E0F1E7}16.67} & \multicolumn{1}{c|}{\cellcolor[HTML]{8CCF9F}66.67} & \multicolumn{1}{c|}{\cellcolor[HTML]{8CCF9F}66.67} & \cellcolor[HTML]{A8DAB7}50    \\ \midrule
National   Energy Administration             & 11                      & \multicolumn{1}{c|}{\cellcolor[HTML]{DEF0E5}18.18} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{DEF0E5}18.18} & \multicolumn{1}{c|}{\cellcolor[HTML]{BFE4CB}36.36} & \multicolumn{1}{c|}{\cellcolor[HTML]{B0DEBE}45.45} & \multicolumn{1}{c|}{\cellcolor[HTML]{BFE4CB}36.36} & \multicolumn{1}{c|}{\cellcolor[HTML]{B0DEBE}45.45} & \cellcolor[HTML]{A1D7B0}54.55 \\ \midrule
National Urban   League                      & 6                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{E0F1E7}16.67} & \multicolumn{1}{c|}{\cellcolor[HTML]{A8DAB7}50}    & \cellcolor[HTML]{C4E6CF}33.33 \\ \midrule
National   Development and Reform Commission & 8                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{93D2A5}62.5}  & \multicolumn{1}{c|}{\cellcolor[HTML]{93D2A5}62.5}  & \cellcolor[HTML]{A8DAB7}50    \\ \midrule
NDRC                                         & 6                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{E0F1E7}16.67} & \multicolumn{1}{c|}{\cellcolor[HTML]{E0F1E7}16.67} & \multicolumn{1}{c|}{\cellcolor[HTML]{E0F1E7}16.67} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     \\ \midrule
ADF                                          & 6                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{A8DAB7}50}    & \multicolumn{1}{c|}{\cellcolor[HTML]{A8DAB7}50}    & \multicolumn{1}{c|}{\cellcolor[HTML]{C4E6CF}33.33} & \multicolumn{1}{c|}{\cellcolor[HTML]{C4E6CF}33.33} & \cellcolor[HTML]{C4E6CF}33.33 \\ \midrule
Australian   Defense Force                   & 4                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{A8DAB7}50}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     \\ \midrule
China                                        & 11                      & \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}90.91} & \multicolumn{1}{c|}{\cellcolor[HTML]{A1D7B0}54.55} & \multicolumn{1}{c|}{\cellcolor[HTML]{73C589}81.82} & \multicolumn{1}{c|}{\cellcolor[HTML]{91D1A3}63.64} & \multicolumn{1}{c|}{\cellcolor[HTML]{A1D7B0}54.55} & \cellcolor[HTML]{82CB96}72.73 & \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}90.91} & \multicolumn{1}{c|}{\cellcolor[HTML]{BFE4CB}36.36} & \multicolumn{1}{c|}{\cellcolor[HTML]{A1D7B0}54.55} & \multicolumn{1}{c|}{\cellcolor[HTML]{A1D7B0}54.55} & \multicolumn{1}{c|}{\cellcolor[HTML]{B0DEBE}45.45} & \cellcolor[HTML]{A1D7B0}54.55 \\ \midrule
Corporate   Library                          & 6                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{E0F1E7}16.67} & \cellcolor[HTML]{8CCF9F}66.67 \\ \midrule
Portland                                     & 5                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{B9E1C5}40}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEFE2}20}    & \multicolumn{1}{c|}{\cellcolor[HTML]{DBEFE2}20}    & \multicolumn{1}{c|}{\cellcolor[HTML]{B9E1C5}40}    & \cellcolor[HTML]{B9E1C5}40    \\ \midrule
Pakistani                                    & 4                       & \multicolumn{1}{c|}{\cellcolor[HTML]{D2EBDB}25}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{A8DAB7}50}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     & \multicolumn{1}{c|}{\cellcolor[HTML]{D2EBDB}25}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \cellcolor[HTML]{FCFCFF}0     \\ \midrule
American                                     & 7                       & \multicolumn{1}{c|}{\cellcolor[HTML]{CCE9D6}28.57} & \multicolumn{1}{c|}{\cellcolor[HTML]{E4F3EB}14.29} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCE9D6}28.57} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{B4DFC1}42.86} & \cellcolor[HTML]{84CC98}71.43 & \multicolumn{1}{c|}{\cellcolor[HTML]{CCE9D6}28.57} & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FCFCFF}0}     & \multicolumn{1}{c|}{\cellcolor[HTML]{E4F3EB}14.29} & \multicolumn{1}{c|}{\cellcolor[HTML]{E4F3EB}14.29} & \cellcolor[HTML]{CCE9D6}28.57 \\ \bottomrule
\end{tabular}
\end{table}
